Optimal least-squares solution to the hand-eye calibration problem

We propose a least-squares formulation to the noisy hand-eye calibration problem using dual-quaternions, and introduce efficient algorithms to find the exact optimal solution, based on analytic properties of the problem, avoiding non-linear optimization. We further present simple analytic approximate solutions which provide remarkably good estimations compared to the exact solution. In addition, we show how to generalize our solution to account for a given extrinsic prior in the cost function. To the best of our knowledge our algorithm is the most efficient approach to optimally solve the hand-eye calibration problem.

==> sections/alternate_convexity_proofs.tex <==
\section{Convexity proof}\label{app:convexity_proof}
{\color{blue}
Let $\lambda_0(\mu)$ be the smallest eigenvalue of the matrix $Z(\mu) = Z_0 + \mu Z_1 - \mu^2 Z_2$ where each $Z_i$ is real symmetric and $Z_0, Z_2$ are positive semidefinite. We want to show that $\lambda_0(\mu)$ is a concave function. Recall that a real-valued function $f(x)$ is concave if and only if 
\begin{align}
    f(\beta x + (1-\beta) y) \geq \beta f(x) + (1-\beta)f(y)
\end{align} 
for any $0\leq \beta\leq 1$ and $x,y\in\mathbb{R}$. For any real symmetric $A,B$ and $0\leq\alpha\leq 1$ we have
\begin{align*}
    \lambda_{\max}(\alpha A + (1-\alpha)B)  &=      \max_{x^2 = 1} x^T(\alpha A + (1-\alpha)B)x
    \\                                      &=      \max_{x^2 = 1} (\alpha x^TAx + (1-\alpha)x^TBx)
    \\                                      &\leq   \alpha\max_{x^2 = 1} x^TAx + (1-\alpha)\max_{x^2 = 1}x^TBx 
    \\                                      &=      \alpha\lambda_{\max}(A) + (1-\alpha)\lambda_{\max}(B)
\end{align*}




\subsection{$\lambda_{\max}(A)$ is increasing in $A$:}
For positive semidefinite (psd) $B$ we have
\begin{align*}
     \lambda_{\max}(A + B)  &=      \max_{x^2 = 1} x^T(A + B)x
     \\                     &=      \max_{x^2 = 1} (x^TAx + x^TBx)
     \\                     &\geq   \max_{x^2 = 1} x^TAx
\end{align*}
since $x^TBx \geq 0$ for any $x$
    
\subsection{$\lambda_{\max} (Z(\mu))$ is convex in $\mu$:}
For $Z(\mu) = Z_0 + \mu Z_1 + \mu^2Z_2$ with $Z_2$ psd we have
\begin{align*}
        &\lambda_{\max} (Z(\alpha \mu + (1-\alpha)\xi))      
        \\ &= \lambda_{\max} (Z_0 + (\alpha \mu + (1-\alpha)\xi) Z_1 + (\alpha \mu + (1-\alpha)\xi)^2 Z_2)    
        \\ &\text{($x\rightarrow x^2$ is convex, $\lambda_{\max}$ is increasing and $Z_2$ is psd):}
\\      &\leq \lambda_{\max} (Z_0 + (\alpha \mu + (1-\alpha)\xi) Z_1 + (\alpha \mu^2 + (1-\alpha)\xi^2) Z_2)
\\      &= \lambda_{\max} (\alpha(Z_0 + \mu Z_1 + \mu^2 Z_2) + (1-\alpha)(Z_0 + \xi Z_1 + \xi^2 Z_2))
\\      &= \lambda_{\max} (\alpha Z(\mu) + (1-\alpha)Z(\xi))
        \\ &\text{($\lambda_{\max}$ is convex):}
\\      &\leq \alpha\lambda_{\max}(Z(\mu)) + (1-\alpha)\lambda_{\max}(Z(\xi))
\end{align*}

\section{Alternate convexity proof}
 Suppose $Z(\mu)$ is a real symmetric $n\times n$ matrix parametrized by $\mu\in\mathbb{R}$. We can then define functions $q_i(\mu)$ and $\lambda_i(\mu)$ implicitly through the eigenvalue problem:
\eq{\label{eq:Zq}
    Z(\mu)q_i(\mu) = \lambda_i(\mu) q_i(\mu)
    } 
with $q_i^T(\mu)q_i(\mu) = 1$ and $\lambda_0(\mu)\leq\ldots\leq\lambda_n(\mu)$. Suppose furthermore that the second derivative $\ddot Z(\mu)$ is negative semidefinite for all $\mu$ and that there are no eigenvalue crossings (points where $\lambda_i(\mu) = \lambda_j(\mu)$ for $i\neq j$). We want to show that the function corresponding to the minimum eigenvalue $\lambda_0(\mu)$ is concave.

We will omit the $\mu$-dependence of $q_i, \lambda_i$ and $Z$ for readability in the remainder of the section. Since there are no eigenvalue crossings we can differentiate (\ref{eq:Zq}) with respect to $\mu$ to get:
\eq{\label{eq:dot}
    \dot Z q_i + Z\dot q_i = \dot\lambda_i q_i + \lambda_i\dot q_i
}
From this we can get an expression for the first derivative of the eigenvalues by multiplying (\ref{eq:dot}) by $q_i^T$ from the left and using $\dot q_i^Tq_i = 0$: 
\eq{\label{eq:lambdadot}
    \dot\lambda_i = q_i^T\dot Zq_i.
}
Taking the derivative of (\ref{eq:lambdadot}) we also get an expression for the second derivative:
\eq{
    \label{eq:lambdaddot}
    \ddot\lambda_i = 2\dot q_i^T\dot Zq_i + q_i^T\ddot Zq_i.
}
Now, note that $q_i^T\ddot Zq_i\leq 0$ for all $i$ since $\ddot Z$ is negative semidefinite. Furthermore, multiplying (\ref{eq:dot}) by $\dot q_i^T$ from the left and grouping terms we get: 
\eq{
    \dot q_i^T\dot Z q_i = -\dot q_i^T(Z -\lambda_i)\dot q_i
}
which, plugging in $i=0$, implies that $\dot q_0^T\dot Z q_0 \leq 0$. Combining these two facts with (\ref{eq:lambdaddot}) we can conclude that $\ddot\lambda_0\leq 0$ for all $\mu$ and thus $\lambda_0$ is a concave function of $\mu$.

A similar argument can also be used to show that $\lambda_n$ is convex if $\ddot Z$ is positive semidefinite for all $\mu$.

\section{Alternate alternate convexity proof}
Suppose $Z(\mu)$ is a real symmetric matrix parametrized by $\mu\in\mathbb{R}$ and that $\ddot Z(\mu)$ is negative semidefinite for all $\mu$. A well known fact is that the smallest eigenvalue $\lambda_0(\mu)$ of $Z(\mu)$ can be written as a minimization problem:
\eq{
    \lambda_0(\mu) = \min_{q^2 = 1} q^TZ(\mu)q.
}
Note that the function $f_q(\mu) = q^TZ(\mu)q$ is concave for fixed $q$ since $\ddot f_q(\mu) = q^T\ddot Z(\mu)q\leq 0$. $\lambda_0(\mu)$ is therefore also concave since it's the minimum over a set of concave functions. 
}
